Cryptography in the Common Haar State Model: Feasibility Results and Separations

Common random string model is a popular model in classical cryptography. We study a quantum analogue of this model called the common Haar state (CHS) model. In this model, every party participating in the cryptographic system receives many copies of one or more i.i.d Haar random states. We study feasibility and limitations of cryptographic primitives in this model and its variants: - We present a construction of pseudorandom function-like states with security against computationally unbounded adversaries, as long as the adversaries only receive (a priori) bounded number of copies. By suitably instantiating the CHS model, we obtain a new approach to construct pseudorandom function-like states in the plain model. - We present separations between pseudorandom function-like states (with super-logarithmic length) and quantum cryptographic primitives, such as interactive key agreement and bit commitment, with classical communication. To show these separations, we prove new results on the indistinguishability of identical versus independent Haar states against LOCC (local operations, classical communication) adversaries.

==> Separations.tex <==
\section{Quantum Black-Box Separation in the QCCC Model} \label{sec:QBB_QCCC}
In this section, we present quantum black-box separations in the \emph{quantum computation classical communication} (QCCC) setting. 

\begin{definition}[QCCC key agreements relative to oracle]
A QCCC key agreement relative to an oracle $\cO$ is a two-party interactive protocol consisting of a pair of uniform QPT oracle algorithms $(\alice,\bob)$, both with oracle access to $\cO$ and with their communication being classical. Let $q = q(\secp)$ be an arbitrary polynomial. $\alice,\bob$ each take as input the security parameter $1^\secp$, ask $q$ queries to the oracle $\cO$, and outputs classical keys $k_\alice\in\bit$ and $k_\bob\in\bit$ respectively.
\begin{itemize}
    \item \textbf{Completeness.} There exists a negligible function $\negl$ such that for all $\secp\in\N$,
    \[
    \Pr\left[
    k_\alice = k_\bob: 
    \substack{ O \gets \cO, \\
    (k_\alice, k_\bob, \tau) \gets \langle \alice^O(1^\secp), \bob^O(1^\secp) \rangle }
    \right] 
    \geq 1 - \negl(\secp),
    \]
    where $\langle\alice,\bob\rangle$ denote the execution of the protocol and $\tau$ is the transcript of the protocol.
    \item \textbf{Statistical Security.} For every computationally unbounded eavesdropper $\eve$ without oracle access to $\cO$,\footnote{Similarly, we relax the security definition.} there exists a negligible function $\negl$ such that for all $\secp\in\N$,
    \[
    \Pr\left[
    k_\eve = k_\bob:
    \substack{ O \gets \cO, \\
    (k_\alice, k_\bob, \tau) \gets \langle \alice^O(1^\secp), \bob^O(1^\secp) \rangle, \\
    k_E \gets \eve(1^\secp,\tau) }
    \right] 
    \leq \frac{1}{2} + \negl(\secp).
    \]
\end{itemize}
\end{definition}

\begin{definition}[QCCC interactive commitments relative to oracle]
A QCCC commitment relative to an oracle $\cO$ is a two-party interactive protocol consisting of a pair of uniform QPT oracle algorithms $(C,R)$, where $C$ is the committer and $R$ is the receiver. Let $q = q(\secp)$ be an arbitrary polynomial. Each of $C$ and $R$ can ask $q$ queries to the oracle $\cO$ and are allowed to communicate classically.
\begin{itemize}
    \item \textbf{Commit phase:} In the (possibly interactive) commit phase, $C$ takes as input the security parameter $1^\secp$ and a bit $b\in\bit$, and $R$ takes as input the security parameter $1^\secp$. We denote the execution of the commit phase by $(\sigma_{CR},\tau) \gets \commit\langle C^\cO(1^\secp,b), R^\cO(1^\secp) \rangle$, where $\sigma_{CR}$ is the joint state of $C$ and $R$ after the commit phase, and $\tau$ denotes the transcript in the commit phase.
    \item \textbf{Reveal phase:} In the (possibly interactive) reveal phase, the output is $\mu\in\set{0,1,\bot}$ indicating the receiver's output bit or abort. We denote the execution of the reveal phase by $\mu \gets \reveal\langle C^\cO, R^\cO, \sigma_{CR}, \tau \rangle$.
\end{itemize}
The scheme satisfies the following conditions.
\begin{itemize}
    \item \textbf{Completeness.} There exists a negligible function $\negl$ such that for all $\secp\in\N$,
    \[
    \Pr\left[
    \mu = b: 
    \substack{ O \gets \cO, \\
    b \gets \bit, \\
    (\sigma_{CR},\tau) \gets \commit\langle C^O(1^\secp,b), R^O(1^\secp) \rangle, \\
    \mu \gets \reveal\langle C^O, R^O, \sigma_{CR}, \tau \rangle, \\
    \mu\in\set{0,1,\bot}
    }
    \right] 
    \geq 1 - \negl(\secp).
    \]
    \item \textbf{Statistical Hiding.} For every computationally unbounded malicious receiver $R^*$ who asks at most $q$ queries, there exists a negligible function $\negl$ such that for all $\secp\in\N$,
    \[
    \Pr\left[
    b' = b:
    \substack{ O \gets \cO, \\
    b \gets \bit, \\
    (\sigma_{CR^*},\tau) \gets \commit\langle C^O(1^\secp,b), {R^*}^O(1^\secp) \rangle, \\
    b' \gets {R^*}^O(\sigma_{R^*}, \tau)
    }
    \right] \leq \frac{1}{2} + \negl(\secp),
    \]
    where $\sigma_{R^*}$ denotes the state obtained by tracing out the committer's part of the state $\sigma_{CR^*}$.
    \item \textbf{Statistical Binding.} For every computationally unbounded malicious committer $C^*$ who asks at most $q$ queries, there exists a negligible function $\negl$ such that for all $\secp\in\N$,
    \[
    \Pr\left[
    \mu = b:
    \substack{ O \gets \cO, \\
    (\sigma_{C^*R},\tau) \gets \commit\langle {C^*}^O(1^\secp), R^O(1^\secp) \rangle, \\
    b \gets \bit, \\
    \mu \gets \reveal\langle {C^*}^O(b), R^O, \sigma_{C^*R}, \tau \rangle
    }
    \right] \leq \frac{1}{2} + \negl(\secp).
    \]
\end{itemize}
\end{definition}

\subsection{The separating oracle}
As is common in black-box impossibility results, we will define oracles relative to which $\omega(\log(\secp))$-PRSs exist while QCCC key agreements and interactive commitments do not. We define the oracle $G := \set{\set{G_k}_{k \in \bit^\secp}}_{\secp\in\N}$ as follows. For every $\secp\in\N$ and $k\in\bit^\secp$, the oracle $G_k$ is a Haar isometry that maps any state $\ket{\psi}$ to $\ket{\psi}\ket{\vartheta_k}$, where $\ket{\vartheta_k}$ is a Haar state of length $n(\secp) = \omega(\log(\secp))$. The existence of $\omega(\log(\secp))$-PRSs relative to $G$ can be proven easily.

\begin{lemma}[$(\secp,\omega(\log(\secp)))$-PRSs exist relative to $G$] \label{lem:oracle_implies_PRS}
There exists a $(\secp,\omega(\log(\secp)))$-PRS generator relative to $G$. In particular, for any polynomial $q(\cdot)$ and any computationally unbounded adversary $\alice^G$ that asks $q(\secp)$ quantum queries to $G$, the distinguishing advantage is negligible.
\end{lemma}
\begin{proof}[Proof sketch]
The proof is similar to the proof of~\cite[Lemma~30]{Kretschmer21}. The implementation of the PRS is simply the oracle $G$: on input $k$, outputs the state $\ket{\vartheta_k}$ generated by $G_k$. The security follows from the hardness of the unstructed search problem~\cite{BBBV97}.
\end{proof}

\subsection{Separating QCCC Key Agreements from $(\secp,\omega(\log(\secp)))$-PRSs}
In this section, we show the quantum black-box separation between QCCC key agreements and $\omega(\log(\secp))$-PRSs. The main idea is very similar to the proof of~\Cref{thm:Imp_QCCC_CHS}: for any protocol interacting with the oracle $G$, we convert it into the one interacting with two \emph{independent} oracles. Hence, the parties can (time-inefficiently) sample their oracle individually and execute the protocol in the plain model. For technical reasons, we only allow the parties to ask \emph{classical} queries to oracles $\set{G_k}_{k\in\bit^\secp}$ on security parameter $1^\secp$ (see~\Cref{remark:QBB} for details). Similarly, from~\Cref{cor:LOCC_repetition}, we will show that doing so will not damage the completeness and security too much. Otherwise, we can construct an LOCC distinguisher $(\alice, \bob)$ with a non-negligible advantage. The extra effort compared to the proof of~\Cref{thm:Imp_QCCC_CHS} is the following: given input states, $(\alice,\bob)$ need to jointly maintain a list $\cL$ of pairs of indices in order to answer the queries consistently, similar to lazy evaluation.

\begin{lemma}[Breaking every $\KA^G$] \label{lem:KA_eve}
For any QCCC key agreement relative to $G$ satisfying completeness and where the parties only make classical queries to $\set{G_k}_{k\in\bit^\secp}$ for every $\secp\in\N$, there exists an eavesdropper (possibly time-inefficient) who breaks the security (and makes no query to $G$).
\end{lemma}
\begin{proof}
Suppose $\KA^G = (P_1^G,P_2^G)$ is a QCCC key agreement relative to $G$ that satisfies completeness. Suppose $P_1$ and $P_2$ each ask $g = g(\secp) = \poly(\secp)$ queries to $G$. We will convert it into a key agreement $\wt{\KA} = (\wt{P_1},\wt{P_2})$ in the plain model. Fix the security parameter. Basically, $\wt{\KA}$ is the same as $\KA^G$ except that $\wt{P_1}$ and $\wt{P_2}$ are respectively interacting with two \emph{independent} oracles $\set{G_k}_{k\in\bit^\secp}$ and $\set{G'_k}_{k\in\bit^\secp}$. Hence, $\wt{P_1}$ and $\wt{P_2}$ first sample their oracles individually and then run $P_1, P_2$.

First, we claim that $\wt{\KA}$ also satisfies completeness. Otherwise, similarly to the proof of~\Cref{thm:Imp_QCCC_CHS},  we construct an LOCC distinguisher $(\alice,\bob)$ for the task in~\Cref{cor:LOCC_repetition} (setting $t = q = 2g$) with a non-negligible advantage as follows:
\begin{enumerate}
    \item $\alice$ and $\bob$ receive input register $(\sfA_1,\sfA_2,\dots,\sfA_{2g})$ and $(\sfB_1,\sfB_2,\dots,\sfB_{2g})$ respectively.
    \item $\alice$ and $\bob$ initialize a list $\cL = \set{(1,\bot),(2,\bot),\dots,(2g,\bot)}$, and runs $P_1^{(\cdot)}, P_2^{(\cdot)}$ as the following steps.
    \item In the $\ell$-th round (suppose it's $\alice$'s round), $\alice$ feeds the message $m_{\ell-1}$ received from $\bob$ in the $(\ell-1)$-th round to $P_1$.\footnote{In the first round (suppose it's $\alice$'s round), $\alice$ simply runs $P_1$ on input the security parameter and $m_0 := \bot$.} Upon receiving $\alice$'s query on $x\in\bit^\secp$, $\alice$ checks if $(i,x)$ is in $\cL$ for some $i\in[2g]$ (\ie whether $x$ has already been queried by $P_1$ or $P_2$). If $(i,x)\in\cL$, then $\alice$ answers the query with a copy of the input state on register $\sfA_i$. Otherwise, $\alice$ finds the first index $j\in[2g]$ with $\bot$ entry, updates it into $(j,x)$, and answers the query with a copy of the input state on register $\sfA_j$. At the end of the round, $P_1$ outputs a classical message $m_\ell$. Then $\alice$ sends $\cL$ and $m_\ell$ to $\bob$.
    \item In $\bob$'s round, $\bob$ does similarly by switching the roles of $P_1$ and $P_2$, and $\alice$ and $\bob$ in the previous step.
    \item At the end of the protocol, $P_1, P_2$ outputs the key $k_{P_1}, k_{P_2}$ respectively.
    \item $\alice$ sends $k_{P_1}$ to $\bob$, and $\bob$ outputs $1$ if $k_{P_1} = k_{P_2}$.
\end{enumerate}
Let $\rho$ and $\sigma$ be defined as in~\Cref{cor:LOCC_repetition}. If the input to $(\alice, \bob)$ is $\rho$, $(\alice, \bob)$ perfectly simulates $\KA^G$. Otherwise, on input $\sigma$, $(\alice, \bob)$ perfectly simulates $\wt{\KA}$. Hence, the advantage of $(\alice, \bob)$ is non-negligible, which contradicts~\Cref{cor:LOCC_repetition} by setting $t = q = 2g = \poly(\secp)$ and $n = \omega(\log(\secp))$.

Next, because of the impossibility of information-theoretic key agreements in the plain model and the fact that $\wt{\KA}$ satisfies completeness, there exists a (possibly time-inefficient) eavesdropper $\wt{\eve}$ that breaks the security of $\wt{\KA}$. We claim that $\wt{\eve}$, without querying $G$, also finds $P_2$'s key in $\KA^G$ with non-negligible advantage. Otherwise, we construct an LOCC distinguisher $(\alice',\bob')$ for the task in~\Cref{cor:LOCC_repetition} (setting $t = q = 2g$) with a non-negligible advantage. $(\alice',\bob')$ runs Step~1 to Step~4 of $(\alice,\bob)$ and obtains $k_{P_1},k_{P_2}$ and the transcript. Then $\bob'$ runs $\wt{\eve}$ on input the transcript and obtains a key $k_\eve$. $\bob'$ outputs $1$ if $k_{P_2} = k_\eve$. Again, the advantage of $(\alice', \bob')$ is non-negligible, which contradicts~\Cref{cor:LOCC_repetition} by setting $t = q = 2g = \poly(\secp)$ and $n = \omega(\log(\secp))$.
\end{proof}

\begin{theorem} \label{thm:QBB_KA}
There does not exist a quantum fully black-box reduction $(C,S)$ from QCCC key agreements to $(\secp,\omega(\log(\secp)))$-PRSs such that on every security parameter $1^\secp$, $C$ only asks classical queries of input length $\secp$ to the $(\secp,\omega(\log(\secp)))$-PRS oracle.
\end{theorem}
\begin{proof}
For the sake of contradiction, suppose $(C,S)$ is a fully black-box reduction satisfying the conditions. Let $\cI$ be the implementation of $(\secp,\omega(\log(\secp)))$-PRSs as stated in the proof of~\Cref{lem:oracle_implies_PRS}. Then $C^\cI$ is a key agreement that satisfies completeness and where the parties only make classical queries to $\set{G_k}_{k\in\bit^\secp}$ for every $\secp\in\N$. From~\Cref{lem:KA_eve}, there exists an adversary $\wt{\eve}$ that breaks the security of the QCCC key agreement $C^\cI$. Then $S^{{\wt{\eve}},\cI}$ by definition breaks the security of the $(\secp,\omega(\log(\secp)))$-PRS $\cI$ by asking polynomially many queries to $\wt{\eve}$ and $\cI$, thus in total polynomial queries to $G$. However, this contradicts~\Cref{lem:oracle_implies_PRS}.
\end{proof}

\subsection{Separating QCCC Interactive Commitments from $(\secp,\omega(\log(\secp)))$-PRSs}
\begin{lemma}[Breaking every $\Com^G$]
For any QCCC interactive commitment relative to $G$ satisfying completeness and where the parties only make classical queries to $\set{G_k}_{k\in\bit^\secp}$ for every $\secp\in\N$, there exists either a malicious sender (possibly time-inefficient) who makes no query and breaks hiding, or a malicious receiver (possibly time-inefficient) who makes no query and breaks binding.
\end{lemma}
\begin{proof}[Proof sketch]
The proof is very similar to that of~\Cref{thm:Imp_QCCC_CHS} and~\Cref{lem:KA_eve}. Suppose $\Com^G = (C^G,R^G)$ is a QCCC interactive commitment relative to $G$ that has a negligible completeness error. Let $g = \poly(\secp)$ denote the number of queries asked by $C$ and $R$. We will convert it into a QCCC interactive commitment $\wt{\Com} = (\wt{C},\wt{R})$ in the plain model. $\wt{\Com}$ is the same as $\Com^G$ except that $\wt{C}$ and $\wt{R}$ are interacting with two \emph{independent} oracles $\set{G_k}_{k\in\bit^\secp}$ and $\set{G'_k}_{k\in\bit^\secp}$. The completeness error of $\wt{\Com}$ is negligible by a similar argument as in the proof of~\Cref{lem:KA_eve}.

From the impossibility of statistically hiding and statistically binding commitments in the plain model, there exists either $\wt{R}^*$ who breaks the statistical hiding or $\wt{C}^*$ who breaks the statistical binding of $\wt{\Com}$. Following the argument in the proof of~\Cref{thm:Imp_QCCC_CHS} and~\Cref{lem:KA_eve}, such $\wt{R}^*$ or $\wt{C}^*$ will break the security of $\Com$ without querying the oracle.
\end{proof}

\begin{theorem} \label{thm:QBB_Com}
There does not exist a quantum fully black-box reduction $(C,S)$ from QCCC interactive commitments to $(\secp,\omega(\log(\secp)))$-PRSs such that on every security parameter $1^\secp$, $C$ only asks classical queries of input length $\secp$ to the $(\secp,\omega(\log(\secp)))$-PRS oracle.
\end{theorem}
\begin{proof}
It is essentially the same as the proof of~\Cref{thm:QBB_KA}.
\end{proof}

\begin{remark} \label{remark:QBB}
\par We compare our results with existing results. Note that our impossibility results only rule out implementations that ask classical queries of length equal to the security parameter to the PRS generator. There exist applications that need to run PRS/PRFS generators in superposition, \eg quantum bit commitments~\cite{MY21}, quantum PKEs~\cite{BGH+23}, etc. However, all of them require quantum communication. It is less obvious how this would be helpful in the QCCC setting. To use the LOCC Haar indistinguishability, we restrict the input length of queries made by the parties in the key agreement. We leave the generalization of the impossibility results as an open problem.
\par Next, since PRS generators can be constructed from one-way functions in a black-box way~\cite{JLS18}, one might wonder whether~\Cref{thm:QBB_KA} is already implied by the classical separation result between key agreements and one-way functions~\cite{IR89,BR09}. In other words, can we prove~\Cref{thm:QBB_KA} by using a (classical) random oracle? We pointed out that all currently known constructions of PRS generators from one-way functions~\cite{JLS18,BS19,BrakerskiS20,GB23,JMW23} require \emph{quantum} oracle access. The impossibility of QCCC key agreements in the quantum random oracle model was studied in~\cite{ACC+22}, where they ruled out \emph{perfectly-complete} key agreements based on a conjecture. However, \Cref{thm:QBB_KA} separates imperfectly-complete key agreements from $\omega(\log(\secp))$-PRSs without relying on any conjecture. Hence, the two results are incomparable.
\end{remark}

\subsection{Extanding the separation results} \label{sec:Extend_QBB_PRFS}
We observe that our technique can also separate QCCC key agreements and commitments from \emph{classically accessible $(\secp,m,n)$-PRFSs with $n = \omega(\log(\secp))$} and $m$ being arbitrary. Recall that currently there is no construction of long-input PRFSs (\ie $m = \omega(\log(\secp))$) from PRSs. Hence, the separation might be strictly stronger. To prove it, we strengthen the separating oracle by increasing the number of oracles as $G = \set{\set{G_{k,x}}_{k,x\in\bit^\secp}}_{\secp\in\N}$. In this way, $G$ can support answering the classical query on key $k$ and input $x$. The rest of the proof is identical to the case of $(\secp,\omega(\log(\secp)))$-PRSs.
